A Survey on Responsible Generative AI: What to Generate and What Not

In recent years, generative AI (GenAI), like large language models and text-to-image models, has received significant attention across various domains. However, ensuring the responsible generation of content by these models is crucial for their real-world applicability. This raises an interesting question: What should responsible GenAI generate, and what should it not? To answer the question, this paper investigates the practical responsible requirements of both textual and visual generative models, outlining five key considerations: generating truthful content, avoiding toxic content, refusing harmful instruction, leaking no training data-related content, and ensuring generated content identifiable. Specifically, we review recent advancements and challenges in addressing these requirements. Besides, we discuss and emphasize the importance of responsible GenAI across healthcare, education, finance, and artificial general intelligence domains. Through a unified perspective on both textual and visual generative models, this paper aims to provide insights into practical safety-related issues and further benefit the community in building responsible GenAI.

==> sections/sec1_intro_writing_sample.tex <==

\section{Introduction}\label{Sec:Introduction}

Generative AI (GenAI) has received remarkable attention recently. Various generative models have been developed in diverse domains, for example, autoregressive large language models~\citep{brown2020language,touvron2023llama} and text-to-image generative models~\citep{saharia2022photorealistic,rombach2022high,betker2023improving}. In real-world applications, the generated contents have to be not only high-quality but also responsible. Thus, this raises the question: What should responsible GenAI generates, and what not?

In this paper, we summarize the responsible requirements of current generative models. Two types of generative models are mainly considered in this work, namely, textual generative models and visual ones. Specifically, textual generative models generate textual responses based on textual or visual inputs, which include autoregressive large language models~\citep{brown2020language,touvron2023llama} and multimodal LLMs~\citep{geminiteam2023gemini,openai2023gpt4}. Similarly, visual generative models are the models that generate images or videos based on textual and visual inputs~\citep{rombach2022high,betker2023improving,sora}.

For both types of generative models, we summarize five responsible requirements for the generated contents. The requirements are not comprehensive, we only review five popular requirements that are important to both academic and industrial communities. Concretely, the five requirements are as follows:

\textbf{1. To generate truthful content.} The generated content is expected to be truthful. However, current generative models could generate content that strays from factual reality or includes fabricated information, which is known as \textit{Hallucination}~\citep{maynez2020faithfulness}. For instance, language models would generate non-fact, and text-to-image models create images with objects that are not specified in the text prompts. Many efforts have been made to identify, elucidate, and tackle the problem of hallucination~\citep{huang2023survey}.

\textbf{2. Not to generate toxic content.} It is well known that both language models and image generation models could generate biased content~\citep{sap2019social,naik2023social}. More recently, with wide applications, it has been found that toxic content could also be generated as responses to end-users. The goal to make generated content unbiased and non-toxic has been intensively explored from various perspectives, e.g., filtering training data and fine-tuning~\citep{ganguli2022red,friedrich2023fair}.


\textbf{3. Not to generate content for harmful instructions.} With or without safety alignment, the current generative AI model can still generate inappropriate content given the adversarial prompts, which is known as \textit{Jailbreak}~\citep{perez2022ignore}. For instance, the textual generative models would output the details for the input prompt 'How to build bombs?' + adversarial prompt. Visual generative models would generate inappropriate images when adversarial text prompts are given~\citep{yang2024sneakyprompt}. Much effort has been made to reveal such vulnerability and defend against these adversarial prompts.


\textbf{4. Not to generate training data-related content.} Recent generative models are often large-scale and have a large number of parameters. Recent research shows that the learned parameters contain the information of training instances. For instance, training text from a language model can be extracted~\citep{carlini2021extracting}, and training images can be synthesized with the corresponding pre-trained text-to-image model~\citep{carlini2023extracting}. How to better extract training data from pre-trained generative models and how to hide the training data information have been intensively studied in our community.

\textbf{5. To Generate identifiable content.} The copyright of generated content is a complicated problem, which requires the knowledge of multiple disciplines. There are multiple levels of copyright problems. One is how to generate detectable content, e.g. with watermarks~\citep{usop2021review}. To attribute the copyright, another intensively studied topic is model attribution~\citep{uchendu2020authorship}. It aims to identify which generative model generates a particular instance.



%Our paper is organized as follows: we recall the preliminary knowledge of GenAI and the vulnerability of deep neural networks in Sec.~\ref{sec:pre}. Sec.~\ref{sec:txtGenAI} summarizes the research of textual generative models on responsible generation, while Sec.~\ref{sec:t2iGenAI} presents the research about responsible visual generation. Besides, we also discuss the application of GenAI in different domains from the perspective of responsible AI in Sec.~\ref{sec:apps}. The involved domains include healthcare, education, finance, and artificial general intelligence. Furthermore, we discuss the challenges and opportunities of responsible GenAI in Sec.~\ref{sec:dis} and conclude our paper in Sec.~\ref{sec:conclu}.

%Our paper differs from related works in the following three points: 1) We present the research topics on responsible GenAI and their recent progress. Especially, we provide a unified perspective for both textual generative models and visual generative models. 2) We summarize the practical safety-related problems that both academics and industry have intensively worked on. 3) We discuss the risks and concerns when applying GenAI to various domains, including general-purpose intelligent systems.















